HTAP Databases: A Survey

Since Gartner coined the term, Hybrid Transactional and Analytical Processing (HTAP), numerous HTAP databases have been proposed to combine transactions with analytics in order to enable real-time data analytics for various data-intensive applications. HTAP databases typically process the mixed workloads of transactions and analytical queries in a unified system by leveraging both a row store and a column store. As there are different storage architectures and processing techniques to satisfy various requirements of diverse applications, it is critical to summarize the pros and cons of these key techniques. This paper offers a comprehensive survey of HTAP databases. We mainly classify state-of-the-art HTAP databases according to four storage architectures: (a) Primary Row Store and In-Memory Column Store; (b) Distributed Row Store and Column Store Replica; (c) Primary Row Store and Distributed In-Memory Column Store; and (d) Primary Column Store and Delta Row Store. We then review the key techniques in HTAP databases, including hybrid workload processing, data organization, data synchronization, query optimization, and resource scheduling. We also discuss existing HTAP benchmarks. Finally, we provide the research challenges and opportunities for HTAP techniques.

==> response/general.tex <==
%!TEX root = ../main.tex
\noindent {\bf Dear Editors and Reviewers},

\vspace{1em}

Thank you for your constructive comments. The responses to the comments are as follows.



==> response/meta.tex <==
%!TEX root = ../main.tex


% \subsection*{Responses to the Associate Editor 2}

% \vspace{-.5em}

% \begin{shaded}
% \noindent \emph{\underline{Summary Comments}: Thank you for your submission to TKDE. However, it is my determination that this paper is out of scope for the readers of TKDE.}
% \end{shaded}

% \stitle{\bfit{Response:}} Thanks for the feedback. We have carefully revised the paper following the reviewers' comments. We summarize the main modifications as follows.

\subsection*{Responses to the Associate Editor (AE)}

\vspace{-.5em}

\begin{shaded}
\noindent \emph{\underline{Summary Comments}: Most comments were addressed in the revision. There is one more minor comment raised by reviewer 3. Please address it.}
\end{shaded}

\stitle{\bfit{Response:}} Thanks for the feedback. We have carefully revised the paper following the reviewers' comments.

==> response/r1.tex <==
\subsection*{Responses to Reviewer 2 (R2)}

\vspace{-.5em}


\begin{shaded}
\noindent \emph{\underline{O1}: "Suppose the total number of updated tuples by the OLTP clients is $U^Q_{TP}$". This definition needs be refined. This number of updated tuples should be defined within a time range. Otherwise, all tuples can be considered "updated" from the very beginning of this database’s initiation.
}
\end{shaded}

\stitle{\bfit{Response:}} We appreciate your comments. We have refined the definition of data freshness as follows: \textit{the data freshness refers to the lag time between the analytics and transactions}. To quantify data freshness, HyBench~\cite{pvldb/HyBench} formally defines the F-Score that takes the maximum value of the timestamp differences between the result sets of the OLAP client and OLTP client. We have revised the description in Section~\ref{subsec:trade-off}.

% Formally, for a query $Q$ that is issued by an OLAP client at time $t_Q$, suppose the total number of updated tuples by the OLTP clients is $U_{\mathit{TP}}^{t_0}$, where $t_0$ is time when the first write transaction is committed. Assume the total number of updated tuples that are accessible by $Q$ is $U_{\mathit{AP}}^{t_Q}$, the data freshness $f_D$ is denoted as: $f_D=\frac{U_{\mathit{AP}}^{t_Q}}{U_{\mathit{TP}}^{t_0}}$.

\begin{shaded}
\noindent \emph{\underline{O2}: “A Trade-off. HTAP databases must balance a trade-off between data freshness and performance isolation”. Since it mentions trade-off between data freshness and performance isolation, I wonder if there is a way to quantify the effectiveness of performance isolation so that we can better evaluate this trade-off.
}
\end{shaded}

\stitle{\bfit{Response:}} Thanks for your comments. To quantify the effectiveness of performance isolation, the degradation percentage~\cite{TiDB2020, TPCTC2014} of transactional/analytical throughput is mostly used. One way of quantifying the performance isolation is to compare the performance between a sequential execution and a hybrid execution with the hybrid workload, the lower the metric is, the better the performance isolation is~\cite{pvldb/HyBench}. Let $W_{\mathit{TP}}$ and $W_{\mathit{AP}}$ denote the performance isolation for OLAP and OLTP, respectively. The definitions are as follows:

\begin{equation}
\label{equ:W_TP}
    W_{\mathit{TP}}= (TPS^{(n,0)} - TPS^{(n,m)}) / TPS^{(n,0)}
\end{equation}


\begin{equation}
\label{equ:W_AP}
   W_{\mathit{AP}}= (QPS^{(0,m)} - QPS^{(n,m)}) / QPS^{(0,m)}
\end{equation}

\noindent where \textit{TPS} is the processed transactions per second, and \textit{QPS} is the processed queries per second. ($n$, $m$) is the configured number of \textit{TP} and \textit{AP} workers.

%We define the minimum value of workload isolation is zero.


\begin{shaded}
\noindent \emph{\underline{O3}: There are still many typos.
}
\end{shaded}

\stitle{\bfit{Response:}} Thanks for your comments. We have fixed all the typos according to the suggestions.

==> response/r2.tex <==
\newpage

\subsection*{Responses to Reviewer 3 (R3)}

\vspace{-.5em}

\begin{shaded}
\noindent \emph{\underline{O1}: I have one minor question regarding the statement "the isolation level does not affect the HTAP techniques." I don't believe this is entirely accurate. While I agree that HTAP techniques are essential for the database regardless of the isolation level, the specific technique may vary slightly, especially concerning how concurrency control is handled.
}
\end{shaded}

\stitle{\bfit{Response:}} Thanks a lot for your comments! You are right, the concurrency control techniques should be different when it comes to different isolation levels. As a result, HTAP techniques may vary slightly because the delta table should adapt to different isolation levels. As similar techniques of concurrency control in OLTP can be applied to HTAP systems, existing HTAP techniques did not discuss these issues. We have revised the description in Section~\ref{subsec:MVCC_HTAP}. 

% Unfortunately, we have not been aware of any HTAP techniques that can adapt to different isolation levels

%Varying the isolation levels can indeed affect the HTAP performance, and a more relaxed isolation level can normally achieve a better throughput. We would like to quote the results reported by HATtrick~\cite{sigmod22/HAPtrick}. As shown in Figure~\ref{fig:isolation_level}, the \textit{x}-axis is TPS for OLTP clients and the \textit{y}-axis is QPS for OLAP clients, and concurrency number varies from 1 to 100. The results indicate that as the concurrency number increases, the serializable isolation level has the lower QPS and TPS compared with that of the read committed isolation level. The experimental results are expected because serializable isolation level will hinder queries and transactions from accessing the data while a transaction has a lock on it. The higher the concurrency number is, the more conflicts incur. 

% The concurrency control (CC) protocols could be optimized concerning HTAP workloads. For instance, to speed up the visibility check process of MVCC-based snapshot isolation, LeanStore~\cite{alhomssi2023scalable} proposed a new protocol that minimizes cross-thread communication for better scalability by using a commit log for each worker. However, we have not been aware of any HTAP techniques that can adapt to different isolation levels. Nevertheless, we agree that the saying that "the isolation level does not affect the HTAP techniques" is not rigorous, a more accurate claim could be "different isolation levels will affect the HTAP performance and different concurrency control techniques should be considered". 

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.95\linewidth]{Figures/HATrick_Isolation.pdf} 
% 	\caption{HTAP performance with different isolation levels}	\label{fig:isolation_level}
% \end{figure}

